A linear-time algorithm and analysis of graph Relative Hausdorff distance

Graph similarity metrics serve far-ranging purposes across many domains in data science. As graph datasets grow in size, scientists need comparative tools that capture meaningful differences, yet are lightweight and scalable. Graph Relative Hausdorff (RH) distance is a promising, recently proposed measure for quantifying degree distribution similarity. In spite of recent interest in RH distance, little is known about its properties. Here, we conduct an algorithmic and analytic study of RH distance. In particular, we provide the first linear-time algorithm for computing RH distance, analyze examples of RH distance between pairs of real-world networks as well as structured families of graphs, and prove several analytic results concerning the range, density, and extremal behavior of RH distance values.

==> RH_SIAM_standalone_final(Aug72019)/RH_SIAM_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{A linear-time algorithm and analysis of graph Relative Hausdorff distance}{S.G. Aksoy, K.E. Nowak, and S.J. Young}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A linear-time algorithm and analysis of graph Relative Hausdorff distance}


% Authors: full names plus addresses.
\author{Sinan G. Aksoy\thanks{Pacific Northwest National Laboratory, Richland, WA, 99352 
  (\email{sinan.aksoy@pnnl.gov}, \email{kathleen.nowak@pnnl.gov}, \email{stephen.young@pnnl.gov}).}
\and Kathleen E. Nowak\footnotemark[2]
\and Stephen J.\ Young\footnotemark[2]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

